RRNet: Towards ReLU-Reduced Neural Network for Two-party Computation Based Private Inference

The proliferation of deep learning (DL) has led to the emergence of privacy and security concerns. To address these issues, secure Two-party computation (2PC) has been proposed as a means of enabling privacy-preserving DL computation. However, in practice, 2PC methods often incur high computation and communication overhead, which can impede their use in large-scale systems. To address this challenge, we introduce RRNet, a systematic framework that aims to jointly reduce the overhead of MPC comparison protocols and accelerate computation through hardware acceleration. Our approach integrates the hardware latency of cryptographic building blocks into the DNN loss function, resulting in improved energy efficiency, accuracy, and security guarantees. Furthermore, we propose a cryptographic hardware scheduler and corresponding performance model for Field Programmable Gate Arrays (FPGAs) to further enhance the efficiency of our framework. Experiments show RRNet achieved a much higher ReLU reduction performance than all SOTA works on CIFAR-10 dataset.

==> sections/1_motivation.tex <==
\section{Motivation}

==> sections/4_main_hardware.tex <==
% \subsection{HW Acceleration Framework Design}
\subsection{\textbf{Operator Modeling and Latency Analysis}}\label{sec:hw-latency}
% \vspace{-4pt}
% \subsection{Cryptographic Operator Latency Modeling}\label{sec:hw_model}
% \begin{figure}[ht]
%     \centering
%       \includegraphics[width=0.5\linewidth]{./Fig/FIG_hw_acc.pdf}
%     \vspace{-5pt}
%   \captionof{figure}{Hardware accelerator structure.}
%     \label{fig:hw_acc}
% % \vspace{-15pt}
% \end{figure}

This section will analyze five different operators: 2PC-ReLU, 2PC-$X^2act$, 2PC-MaxPool, 2PC-AvgPool, and 2PC-Conv. Therefore, they require $(1, n)$-OT (noted as \textbf{OT flow} block to implement  2PC comparison flows. Batch normalization can be fused into the convolution layer and it's not listed. %in Fig.~\ref{fig:ReLU-ot} and~\ref{fig:MaxPool-ot}).

% \subsection{Operator Modeling and Latency Analysis}\label{sec:hw-latency}

% Before discussing the \textit{latency} evaluation of each operator, we need to introduce the basic hardware setting of an accelerator. 
% % As shown in Fig.~\ref{fig:hw_acc}, 
% The FPGA-based hardware includes three modules. The ping-pong buffer-based \textbf{LOAD/STORE} modules buffer the input/output data from/to external memory, e.g., DRAM. The compute kernels (\textbf{CMPs/COMMs}) implement processing elements (PEs) for 2PC-ReLU, 2PC-$X^2act$, 2PC-MaxPool, 2PC-AvgPool, or 2PC-Conv. Since batch normalization can be fused into convolution layer, so it's not listed. 
%as a separate operator. 
%Specifically, the optimization target of each kernel is the initiation interval ($II$), which represents the number of clock cycles between two continuous data inputs. The ideal optimized $II$ is equal to 1, meaning that the computation is fully pipelined. To achieve this goal, the data transmission protocol between load module, compute kernel, and store module should be stream-based protocols, such as AXI-stream or FIFO. 


% While the intra-chip communication is stream-based, the inter-chip communication, such as between FPGA on-chip buffer and the external DRAM, uses standard AXI protocol. With the fact that the stream-based protocol is much faster than standard AXI, the bottleneck of the performance appears at the standard AXI protocol.
% We can observe the transmission protocols between each module, where the bottleneck of the performance appears at the external memory to the FPGA on-chip buffer. The \textbf{CMPs/COMMs} implements when the LOAD module has data, and stream-based protocol is much faster than standard AXI. 
% We model the communication latency based on the data transmission between LOAD/STORE module and the DRAM. This latency is related to the bandwidth of the router ($Rt_{bw}$) and the internet ($Nt_{bw}$), communication channel build time ($T_{bc}$), and communication data size ($N_d$). Thus, the data communication latency ($COMM$) can be represented as Eq.~\ref{eq:comm_i}
%  \begin{equation}\label{eq:comm_i}
%      COMM = T_{bc} + \frac{N_d}{\min\{Nt_{bw}, Rt_{bw}\}}
%  \end{equation}
% % For the CMPs timing as shown in Fig. \ref{fig:hw_acc}, the $II$ is optimized to 1, so that the acceleration is fully pipelined. Hence, we can refer to the LOAD/STORE module to build the hardware computing latency ($CMP$).
% % CMPs Timing, where one LOAD/STORE/CMP block represents the load/store and kernel compute instruction. 
% The load/store time is related to the input/output data size, so the $CMP$ equals to the ping/pong buffer size. In addition, large-sized data need repeated instructions, i.e., multiple load-CMP-store stages. For different operators, we have different dataflow estimations, which will be discussed in Sec.~\ref{sec:hw-latency}. 
% Finally, the hardware latency ($HW$) is the summation of the hardware computing latency ($CMP$) and the communication latency $COMM$. 
 

% \subsubsection{\textbf{2PC Polynomial Activation Function}}
% In this work, we propose a hardware friendly trainable polynomial activation function for cryptographic neural network. The second order polynomial activation function is shown in Eq.~\ref{eq:x2act}, $w_1$, $w_2$ and $b$ are all trainable parameters. During inference, we use equivalent form Eq.~\ref{eq:x2act_infe} of the proposed activation and incorporate $w_1'$ and $b_1'$ into the convolution or linear layers' parameters. Thus, the proposed activation only requires a square operation during the inference process. The square operation follows same computation steps with secret-share matrix Hadamard product. 
% \begin{equation}\label{eq:x2act}
% \delta(x) = w_1 x^2 + w_2 x + b
% \end{equation}
% \begin{equation}\label{eq:x2act_infe}
% \delta(x) = (w_1' x + b_1')^2 + b_2' = x'^2 + b_2'
% \end{equation}

% \subsection{Operator Modeling and Latency Analysis}\label{sec:hw-latency}
\begin{figure}[h]
    \centering
      \includegraphics[width=0.8\linewidth]{./Fig/Fig_hw_ot.pdf}
    % \vspace{-5pt}
  \captionof{figure}{Processing Steps of \textbf{2PC-OT} flow.}
    \label{fig:ot}
% \vspace{-15pt}
\end{figure}



% As discussed in Section~\ref{sec:2PC-compare}, the non-linear operator requires 2PC comparison implementation. In this section, we discussed the detail implementations of $(1, n)$-OT (noted as \textbf{OT flow} block) and provide a performance model to predict the 2PC comparison based operator overhead on FPGA platform. 

\subsubsection{2PC-OT Processing Flow} While OT-based comparison protocol has been discussed in~\cite{kilian1988founding}, we hereby provide other communication detail as shown in Fig.~\ref{fig:ot}. 
%All computation is based on extensive power and XOR operation on an unsigned integer ring. 
Assume both servers have a shared prime number $m$, one generator ($g$) selected from the finite space $\mathbb{Z}_m$, and an \textbf{index} list with $L$ length. As we adopt 2-bit part, the length of \textbf{index} list is $L=4$. 
%Furthermore, we consider 32-bit data and local area network (LAN) to model our 2PC operators in accordance with our experimental evaluation as shown in Sec.~\ref{sec:eval}. 

\noindent\textbf{\textcircled{1}} \textbf{Server 0} ($S_0$) generates a random integer $rd_{s_0}$, and compute mask number $S$ with $S = g^{rd_{S_0}}\ mod\ m$, then shares $S$ with the Server 1 ($S_1$). 
% We only need to consider communication ($COMM_1$) latency in Eq.~\ref{eq:COMM_1}, as computation ($CMP_1$) latency is trivial.
% \vspace{-4pt}
% \begin{equation}\label{eq:COMM_1}
%     COMM_1 = T_{bc} + \frac{32}{Rt_{bw}}
% \vspace{-4pt}
% \end{equation}
We consider communication ($COMM_1$) latency as $COMM_1 = T_{bc} + \frac{32}{Rt_{bw}}$. % since computation ($CMP_1$) latency is trivial.
% \vspace{-4pt}
% \begin{equation}\label{eq:COMM_1}
%     COMM_1 = T_{bc} + \frac{32}{Rt_{bw}}
% \vspace{-4pt}
% \end{equation}

\noindent\textbf{\textcircled{2}} \textbf{Server 1} ($S_1$) received $S$, and generates $\bm{R}$ list based on $S_1$'s 32-bit dataset $\bm{M_1}$, and then send them to $S_0$. %Each element of $\bm{M_1}$ is split into $U = 16$ parts, thus each part is with 2 bits. 
    %We can find the message index through a function $b2d(\cdot) + 1$, where $b2d$ is a function transferring a binary number ($l$) to the decimal value, For example with \text{2'b10} as the input, the index output is $b2d(\text{2'b10}) + 1 = 3$. Meanwhile, $S_1$ generates a list of random number $\bm{rd_{S_1}}(u)$, it has the same size as $U = 16$. Thus, $\bm{R}(y, u) = (S^{b2d(\bm{M_1}(y, u)) + 1}\ mod\ m) \oplus (g^{\bm{rd_{S_1}}(u)}\ mod\ m)$, where $y$ represents the value in $\bm{M_1}$ dataset.
    % As we consider the DNN application, we define the input of this OT flow as 2D input feature maps in multiple channels with size $FI \times FI \times IC$, assuming the input feature is square with size $FI \times FI$ and $IC$ denotes the input channel. Since the datatype of this feature map in 32-bit, we can calculate the data size as $32 \times FI^2 \times IC$ bits. During the computation, FPGA can enable the parallelism, so that multiple data can be processed in parallel and pipelining. We denote the computational parallelism as $PP$, so the input length of $\bm{R}$ list is $\frac{32 \times FI^2 \times IC}{PP}$, and the output length is $\frac{32 \times 16 \times FI^2 \times IC}{PP}$. The store time is 16 times the load time for our hardware design, because we split each value into 16 parts. The $CMP_2$ is calculated as shown in Eq.~\ref{eq:CMP_2}, where $freq$ is the execution frequency of the FPGA. Besides, the $COMM_2$ is shown in Eq.~\ref{eq:COMM_2}.
%Assuming the input feature is square with size $FI$ and $IC$ denotes the input channel, and we denote the computational parallelism as $PP$. 
The $CMP_2$ is modeled as Eq.~\ref{eq:CMP_2}, and $COMM_2$ is modeled as Eq.~\ref{eq:COMM_2}. 
% \vspace{-3pt}
\begin{equation}\label{eq:CMP_2}
    CMP_2 = \frac{32 \times 17 \times FI^2 \times IC}{PP \times freq}
    % \vspace{-3pt}
\end{equation}   
\begin{equation}\label{eq:COMM_2}
    COMM_2 = T_{bc} + \frac{32 \times 16 \times FI^2 \times IC}{Rt_{bw}}
    % \vspace{-3pt}
\end{equation}

\noindent\textbf{\textcircled{3}} \textbf{Server 0} ($S_0$) received $\bm{R}$, it will first generate the encryption $\bm{key_0}(y,u) = \bm{R}(y,u)\oplus (S^{b2d(\bm{M_1}(y, u)) + 1}\ mod\ m)^{rd_{S_0}}\ mod\ m$. The $S_0$ also generates is comparison matrix for it's $\bm{M_0}$ with 32-bit datatype and $U = 16$ parts, thus the matrix size for each value ($x$) is $4 \times 16$. The encrypted $Enc(\bm{M_0}(x,u))=\bm{M_0}(x,u)\oplus \bm{key_0}(y,u)$ will be sent to $S_1$. The $COMM_3$ of this step is shown in Eq.~\ref{eq:COMM_3}, and $CMP_3$ can be estimated as Eq.~\ref{eq:CMP_3}. 
\vspace{-3pt}
\begin{equation}\label{eq:CMP_3}
    CMP_3 = \frac{32 \times (17 + (4 \times 16)) \times FI^2 \times IC}{PP \times freq}
    % \vspace{-3pt}
\end{equation}    
\begin{equation}\label{eq:COMM_3}
    COMM_3 = T_{bc} + \frac{32 \times 4 \times 16 \times FI^2 \times IC}{Rt_{bw}}
    % \vspace{-3pt}
\end{equation}

\noindent\textbf{\textcircled{4}} \textbf{Server 1} ($S_1$) decodes the interested encrypted massage by $\bm{key_1} = S^{rd_{S_0}}\ mod\ m$ in the final step. 
%The comparison result will be formulated in a signal bit mask matrix $\bm{T}$ with size $FI^2 \times IC$ and shared with $S_0$. 
The $CMP_4$ and $COMM_4$ are calculated as following:
% \vspace{-5pt}
\begin{equation}\label{eq:CMP_4}
    CMP_4 = \frac{((32 \times 4 \times 16) + 1) \times FI^2 \times IC}{PP \times freq}
    % \vspace{-5pt}
\end{equation}    
\begin{equation}\label{eq:COMM_4}
    COMM_4 = T_{bc} + \frac{FI^2 \times IC}{Rt_{bw}}
    % \vspace{-5pt}
\end{equation}




% \begin{figure}[b]
%     \centering
%       \includegraphics[width=0.75\linewidth]{./Fig/FIG_hw_ReLU.pdf}
%     % \vspace{-5pt}
%   \captionof{figure}{2PC-ReLU flow.}
%     \label{fig:ReLU-ot}
% % \vspace{-15pt}
% \end{figure}

\subsubsection{2PC-ReLU Operator} 2PC-ReLU requires 2PC-OT flow. %If we implement it in two-party manner, the comparison of $x$ v.s. "0" will turn into the comparison between $ x_{S_0}$ and $-x_{S_1}$, as $x = x_{S_0} + x_{S_1}$. 
%One OT flow can directly obtain the 2PC-ReLU task. 
%With a hardware parameter setting of $[T_{bc}, Rt_{bw}, FI, IC, PP, freq]$ 
2PC-ReLU latency ($Lat_{2PC-ReLu}$) model is given in Eq.~\ref{eq:LtReLU}.
\begin{equation}\label{eq:LtReLU}
    Lat_{2PC-ReLu} = \sum_{i = 2}^{4}CMP_i + \sum_{j = 1}^{4}COMM_j
\end{equation}


\subsubsection{2PC-MaxPool Operator} Original MaxPool function is shown in Eq. \ref{eq:org_maxpool}. The 2PC-MaxPool uses OT flow comparison, and the latency model is shown in Eq.~\ref{eq:LtMax}.
%, where the $out(n,c,h,w)$ is the maximum value of partial inputs normalized by kernel, which is related to the kernel size $(K_h, K_w)$ and stride $(S_h, S_w)$. 

% \begin{figure}[t]
%     \centering
%       \includegraphics[width=0.75\linewidth]{./Fig/FIG_hw_MaxPool.pdf}
%     % \vspace{-5pt}
%   \captionof{figure}{2PC-MaxPool flow.}
%     \label{fig:MaxPool-ot}
% \vspace{-5pt}
% \end{figure}

% \begin{equation}\label{eq:org_maxpool}
%     out(n, c, h, w) = \max_{\substack{
% k_h \in [0, K_h -1] \\
% k_w \in [0, K_w -1]\\
% }} in(n, c, hS_h + k_h, wS_w + k_w )
% \end{equation}

% \vspace{-10pt}
\begin{equation}\label{eq:org_maxpool}
    out = \max_{\substack{
k_h \in [0, K_h -1] \\
k_w \in [0, K_w -1]\\
}} in(n, c, hS_h + k_h, wS_w + k_w )
% \vspace{-0pt}
\end{equation}

% \begin{equation}\label{eq:LtMax}
%     Lat_{2PC-MaxPool} = \frac{3}{4} (\sum_{i = 2}^{4}CMP_i + \sum_{j = 1}^{4}COMM_j + 3T_{bc})
% \end{equation}
% \vspace{-8pt}
\begin{equation}\label{eq:LtMax}
    Lat_{2PC-MaxPool} = \sum_{i = 2}^{4}CMP_i + \sum_{j = 1}^{4}COMM_j + 3T_{bc}
\end{equation}

% \begin{figure}[t]
%     \centering
%       \includegraphics[width=1\linewidth]{./Fig/Fig_hw_ot.pdf}
%     \vspace{-16pt}
%   \captionof{figure}{Processing Steps of \textbf{2PC-OT} flow.}
%     \label{fig:ot}
%     \vspace{-18pt}
% % \vspace{-15pt}
% \end{figure}


\subsubsection{2PC-$X^2$act Operator} The original $X^2act$ has been shown in Eq.~\ref{eq:x2act}. 
The $X^2act$ needs a ciphertext square operation and 2 ciphertext-plaintext multiplication operations. The basic protocol is demonstrated in Sec.~\ref{sec:poly}. 
%Starting from the input side, 2PC needs to exchange the masked secret-shared data in the first step to prepare $E$. For each server, five inputs join the square computation, and then the scaling is conducted. Thus, 
%The latency of computation and communication can be modeled as: $CMP_{x^2} = \frac{2 \times FI^2 \times IC}{PP \times freq} $ and $ COMM_{x^2} = T_{bc} + \frac{32 \times FI^2 \times IC}{Rt_{bw}}$. 
The latency model of 2PC-$X^2$act ($Lat_{2PC-X^2act}$) is shown in Eq.~\ref{eq:LtX2}.
% \vspace{-4pt}
\begin{equation}\label{eq:LtX2}
    Lat_{2PC-X^2act} = CMP_{x^2} + 2 \times COMM_{x^2}
% \vspace{-4pt}
\end{equation}

\subsubsection{2PC-AvgPool Operator} The 2PC-AvgPool operator only involves addition and scaling, the latency is 
% \vspace{-4pt}
\begin{equation}
    Lat_{2PC-AvgPool} = \frac{2 \times FI^2 \times IC}{PP \times freq}%\frac{5}{freq}
% \vspace{-4pt}
\end{equation}

\subsubsection{2PC-Conv Operator} The 2PC-Conv operator involves multiplication between ciphertext, and the basic computation and communication pattern are given Sec.~\ref{sec:poly}. The computation part follows tiled architecture implementation \cite{zhang2015optimizing}. 
%and the latency of load/store operations are hidden using coarse-grained pipeline execution. 
%There are four tiling parameters ($Tm$, $Tn$, $Tc$, $Tr$) that correspond to the input channel, output channel, column, and row tile. Tiling parameters can be adjusted according to memory bandwidth and on-chip resources to reduce the communication-to-computation (CTC) ratio and achieve better performance. 
%Assuming we can meet the computation roof by adjusting tiling parameters, the latency of the 2PC-Conv computation part can be estimated as $CMP_{Conv} = \frac{3 \times K \times K \times FO^2 \times IC \times OC}{PP \times freq}$, where $K$ is the convolution kernel size. The communication latency is modeled as $ COMM_{Conv} = T_{bc} + \frac{32 \times FI^2 \times IC}{Rt_{bw}}$. 
The latency of 2PC-Conv is given in Eq.~\ref{eq:Ltconv}. 
\begin{equation}\label{eq:Ltconv}
    Lat_{2PC-Conv} = CMP_{Conv} + 2 \times COMM_{Conv}
\end{equation}

% \subsubsection{\textit{2P-OT} Flow Based Operator} There are 2 main %non polynomial 
% operations in DNN which requries \textit{2P-OT} Flow: \textbf{2P-ReLU} and \textbf{2P-Maxpool}. 

% \noindent\textbf{2P-ReLU:} The ReLU activation $ReLu(x)=max(0,x)$ requires the comparison between original pixel value with 0. However, the recover and compare is not secure. In this work, we compare the shared value $x_{S_0}$ and $-x_{S_1}$ instead, and generate the ReLU operation mask based on \textit{2P-OT} flow. A example of \textbf{2P-ReLU} is given in Fig.~\ref{fig:ReLU-ot}. 

% \noindent\textbf{2P-MaxPool.} MaxPool function with kernel size $(K_h, K_w)$ and stride $(S_h, S_w)$ can be found in Eq. \ref{eq:org_maxpool}. The \textit{2P-MaxPool} requires $NR$ number of reduction step given in Eq. \ref{eq:reduce_stp}. An \textit{2P-MaxPool} with 2*2 kernel size example is given Fig.~\ref{fig:MaxPool-ot}, the nearby 2 pixel value will be compared and reduced in each \textit{2P-OT} flow. 
% \begin{equation}\label{eq:org_maxpool}
% \small
%     out(n, c, h, w) = \max_{\substack{
% k_h \in [0, K_h -1] \\
% k_w \in [0, K_w -1]\\
% }} in(n, c, hS_h + m, wS_w + n )
% \end{equation}
% \begin{equation}\label{eq:reduce_stp}
% \small
%     NR = \lceil\log_2(K_w + K_h)\rceil
% \end{equation}


% \subsubsection {Modeling and Timing Analysis}
% \textcolor{red}{@Yukui, rewrite for 2P-ReLU and 2P-MaxPool modeling}
% There are three time consumption in each non-linear operator. The first two are OT data preparing time and data transmission time, which are denoted as $T_{pre}(\cdot)$ and $T_{dt} (\cdot)$ respectively. They have a relationship with the output size, denoted as $N \times C \times H \times W$. The communication channel handshaking time is a constant $T_{cb}$ for each connection, which depends on the communication protocol and networks types (WAN or LAN). The time consumption for 2P-ReLU is $T_{pre}(N,C,H,W) + T_{dt}(N,C,H,W) + T_{cb}$ and 2P-MaxPool execution time repesents as $T_{pre}(N,C,H,W) + (1-\frac{1}{K_w + K_h})\times T_{dt}(N,C,H,W) + NR \times T_{cb}$.







==> sections/4_post_training_finetune.tex <==
\subsection{Post Search Training Pipeline}
\label{sec:posttraining}

\subsubsection{Polynomial Architecture Training}
To further enhance the model performance, we adopt the transfer learning method \cite{zhuang2020comprehensive} for general weights initialization and \textbf{STPAI} for polynomial weights. After the appropriate model architecture is found from the NAS framework, we load the pre-trained weight parameters for the backbone model and task to target model architecture. 


\begin{figure} [h]
\centering
\includegraphics[width = 0.8\linewidth]{Fig/Fig_finetune.pdf}
\caption{Fine-grained replacement policy.}
% \cw{(i)For consistency purpose, Organization A, B should be computing server A, B. (ii) I suggest to remove Organization C from the figure.}}
\label{fig:finetune}
% \vspace{-2pt}
\end{figure}

However, we observed that for large models on large datasets, such as ResNet50 on ImageNet, the polynomial function may still lead to instability during the training process. As such, we use a more fine-grained replacement policy shown in Fig.~\ref{fig:finetune}. The replacement ratio $s$ indicates how much the target model layer structure replaces the baseline model layers structure. We follow two iterative steps in training to stabilize the process: parameter update using SGD~\cite{amari1993backpropagation} and s increment.
The experiment shows that the post-search training pipeline, which combines transfer learning, \textbf{STPAI}, and fine-grained replacement policy avoids the gradient explosion and achieves a high model accuracy. 

==> sections/5_quantization.tex <==
\subsubsection{Fixed Point$\Leftrightarrow$Integer Encoding Conversion}
\label{sec:quan}

We use fixed point encoding to represent numbers in order 2PC-based inference framework. Assume the original float point number is $x$, and the fixed point counterpart is $\nint{x \cdot S}$, where $S = 2^L$ corresponds to $L$ bits fixed point decimal precision. For each multiplication, the fixed point intermediate result needs to be divided by the scaling factor to maintain the correct scaling. However, the division (truncation) process may lead to another wrap-around error \cite{mohassel2017secureml, wagh2018securenn, knott2021crypten}, and such error is a notorious phenomenon for multi-party computation. In the 2PC setup, the wrap-around error can be estimated as $\frac{\nint{x \cdot S}}{2^b}$, where b is the ring size during evaluation. The ring size plays an important role in the performance of 2PC-based PI, and it needs to be maintained as low as possible. We can either reduce the $x \cdot S$ value or increase the ring size to mitigate the truncation error probability.

In the 2PC-Conv operator, there are $K\times K \times IC$ multiplication results accumulated together for a single output pixel. Thus output scaling of the 2PC-Conv operator will have the highest truncation error probability. 
In order to mitigate the wrap-around without increasing the ring size, we propose to regulate the $\nint{x \cdot S}$ value during evaluation by fixed point$\Leftrightarrow$integer encoding transformation for the 2PC-Conv operator. 

\textbf{Encoding transformation for error mitigation.} Note that the parameter of the convolution layer and the following batch normalization layer are fused to reduce the ciphertext multiplication overhead. We perform a running mean estimation with 0.98 momentum for max absolute activation values estimation ($m_a = max \lvert a \rvert$), and utilizes this information for activation scaling. A similar estimation is also applied to weight, and the scaling is ($m_w = max \lvert w \rvert$). If we constraint the number of bit for plaintext input and weight to q bit, the overall scaling of activation and weight are donated by $\omega_a = \frac{2^q}{m_a}$ and $\omega_w = \frac{2^q}{m_w}$. Prior to 2PC-Conv evaluation, activation and weight are multiplied by $\omega_w$ and $\omega_a$ scaling to reduce the absolute input value. After 2PC-Conv evaluation, the result is divided by $\omega_a \cdot \omega_w$ to recover the originally fixed point encoding. We further adapt a training framework similar to HAWQ~\cite{yao2021hawq} to retain the accuracy of the fixed Point$\Leftrightarrow$Integer encoding transformation. 

% \begin{equation}\label{eq:quant_activiation}
% \small
% q_a=Int(\tfrac{a}{\omega_a})=Int(\tfrac{\omega_w\omega_h}{\omega_a}(q_w \otimes q_h + q_{bias}))
% \end{equation}
% \vspace{-5pt}
% \begin{equation}\label{eq:dn_function}
% \small
% I_m/2^{I_e}=DN(\omega_w\omega_h/\omega_a)
% \end{equation}
% \vspace{-2pt}



% \begin{equation}\label{eq:quant-act}
% \small
% \delta(x) = (w_1' x + b_1')^2 + b_2' = x'^2 + b_2'
% \end{equation}

% \begin{equation}
% \small
% \begin{aligned}
% \label{eq:bnrequant}
% % BNReQuan(q_w*q_h) &= Int(\tfrac{S_wS_h}{S_a}\cdot \beta \tfrac{(q_w*q_h)-\mu }{\sigma }+\gamma )  \\
% % &=Int(\tfrac{\beta S_wS_h}{\sigma S_a }\cdot (q_w*q_h)+(\gamma -\tfrac{\beta\mu }{\sigma S_a}))
% BNReQuan(& q_w\otimes  q_h) = Int((\beta\tfrac{\omega_w\omega_h(q_w\otimes q_h)-\mu }{\sigma }+\gamma)/{\omega_a} ) \\
% &=Int(\tfrac{\beta \omega_w\omega_h}{\sigma \omega_a }\cdot (q_w\otimes q_h)+(\frac{\gamma}{\omega_a}  -\tfrac{\beta\mu }{\sigma \omega_a})) \\
% &=DN(\tfrac{\beta \omega_w\omega_h}{\sigma \omega_a })[{(q_w\otimes q_h)+q_{\overline{bias}}} ]  \\
% &=I_m'/2^{I_e'}[{(q_w\otimes q_h)+q_{\overline{bias}}} ]
% \end{aligned}
% \end{equation}

% \textcolor{red}{delete}
% \textbf{Activation Function quantization}
% For the full precision training, Eq.~\ref{eq:x2act} is used for forward and backward propagation to make sure the convergence of DNN model. After full precision training is done, the Eq.~\ref{eq:x2act_infe} can be adopted to conduct post-training quantization. 

% Eq.~\ref{eq:bnrequant} is used for combined quantization of both DNN layers and the following batch normalization. Using similar method, the parameter of $X^2act$ ($w_1'$ and $b_2'$) in Eq.~\ref{eq:x2act_infe} can also be combined into DNN layers following Eq.\ref{eq:bnrequant}. $w_1'$ and $b_2'$ are obtained from Eq.~\ref{eq:x2act_w_b}. 

% For $X^2act$, the output of equivalent Eq.\ref{eq:bnrequant} is constrained into 8 bit number again and the thus we quantize the $X^2act$ from Eq.~\ref{eq:x2act_infe} ($sign(w_1) \cdot x'^2 + b_2'$) into Eq.~\ref{eq:x2act_quan}. In Eq.~\ref{eq:x2act_quan}, $\omega$ donates the Hadamard product. Output of activation function $q_o$ is then fed into next DNN layer. 


% \begin{equation}
% \small
% \begin{aligned}
% \label{eq:x2act_quan}
% q_o = Int(\tfrac{o}{\omega_o}) = Int(\tfrac{\omega_a^2}{\omega_o}(sign(w_1) \cdot q_a \odot q_a + q_{b_2'}))
% \end{aligned}
% \end{equation}


\textbf{Truncation error case study.}
Assuming we use the ring size as 32 bits, we constrain the plaintext of convolutional layer input activation and weight into 8 bits during evaluation. We show an example of value distribution profiling of 2PC-Conv output for the VGG16 model (with all ReLU) on CIFAR-10 for 8 bits plaintext input scheme. The absolute mean (AbsMean) value are used to estimated the $|x|/2^{32}$ truncation error probability \cite{knott2021crypten}, where $32$ is the ring size. 

\begin{table}[t]
\caption{Error probability analysis for VGG-16 layers}
% \scriptsize

\centering
\resizebox{\linewidth}{!}{
\label{tab:error_prob}
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
Layer           & 1      & 2      & 3      & 4      & 5      & 6      & 7     \\ \hline
AbsMean         & 13,051 & 8,910  & 3,021  & 13,831 & 5,628  & 11,114 & 4,134 \\ \hline
Error Prob ($\times 10^{-6}$) & 3.04  & 2.07  & 0.70  & 3.2  & 1.33  & 2.58  & 0.98 \\ \hline
Layer           & 8      & 9      & 10     & 11     & 12     & 13     &       \\ \hline
AbsMean         & 7,062  & 31,744 & 45,320 & 42,155 & 40,985 & 41,571 &       \\ \hline
Error Prob ($\times 10^{-6}$) & 1.64  & 7.42   & 10.55   & 0.98  & 0.95  & 0.97  &       \\ \hline
\end{tabular}
}

\end{table}

The layer-wise AbsMean and corresponding probability for truncation error is shown is given in Table~\ref{tab:error_prob}, where the truncation error probability ranges from $7\times 10^{-7}$ to $1.055\times 10^{-5}$. 
Activation absolute value distribution is shown in Fig.~\ref{fig:act_dist}. The distribution indicates that most values are near the layer-wise mean. Thus the error probability is similar within the layer. 
% The profiling 
Results show that with the proposed fixed point$\Leftrightarrow$integer workflow setup and bit-width selection, truncation error will be negligible and have little effect on prediction accuracy. 
%The profiling shows that most values falls into range of XX to XX, and has a mean value of XX. It indicates that for a 20-bit ring size, there will only be XX error probability for ring size overflow and is negligible. 



\begin{figure}[t!]
    \centering
    %   \includegraphics[width=0.9\linewidth]{./Fig/cifar10_act_dist.pdf}
      \includegraphics[width=0.6\linewidth]{./Fig/cifar10_act_dist_3.pdf}
  \captionof{figure}{Feature map value distribution for VGG16.
%   on CIFAR-10 
  }
    \label{fig:act_dist}
\end{figure}

==> sections/7_related_work.tex <==
\section{Related Work}


% \subsection{Hardware Aware Neural Architecture Search}

% This section describes our DIAN framework. We first provide
% an overview and the problem formulation, and then DIAN’s
% co-search algorithm, followed by DIAN’s two search engines
% and the proposed generic accelerator space.

% In this section, we will present the proposed framework. We will use the NAS discussed in [16] as the backbone framework and FPGA as the hardware platform to demonstrate our concept. It can be integrated with any existing NAS techniques [16], [8], [17], [18] or extended to incorporate other hardware platforms.

% In this section, we provide a overview of 

% formulate the problem 


% \subsection{Challenges in Secure MPC based PI}
Secure MPC, a cryptographic technique, is used to allow multiple parties to jointly and securely perform a function while keeping each party's inputs private. MPC is capable of providing security guarantees as robust as those achievable by trusted third parties~\cite{canetti2001universally}. 
% For instance, with absolutely no information is leaked other than that can be obtained from the expected function outputs.
% Researchers have been using MPC to build secure, privacy-preserving DNN frameworks.
% \textcolor{blue}{Drawback of MPC} \\
% Although secure MPC for PPML and PI has smaller encryption overhead compared to HE based method \cite{lee2022privacy, huang2022cheetah}, it still comes with a order of magnitude higher computation \& communication overhead during encrypted evaluation compared to plaintext evaluation. The encryption overhead introduced by secure MPC protocol could potentially prohibit the popularity and the adoption of PPML in MLaaS application, especially for edge platforms such as mobile or IoT with limited resources. Thus, designing a scalable and provably secure DNN framework is considerably challenging, especially given that the current DNN model gets bigger and more complex. 
% \textcolor{blue}{Bottleneck of MPC} \\
% To reduce the latency and memory footprint overhead of secure MPC based PPML, we firstly need to identify the design bottleneck of MPC protocol in DNN inference. 
The DNN operators can be classified into 2 categories: linear operators and non-linear operators. Linear operator includes fully connected (FC) layer, convolutional layer and average pooling operator. Linear operator is evaluated based on encrypted multiplication using random Beaver triples \cite{beaver1991efficient} and addition, and it has a fair cost in secure MPC based PI. However, the non-linear operators, such as ReLU and sigmoid, requires garbled circuit \cite{knott2021crypten} based secure comparison protocol implementation, and the protocol normally leads to several order of magnitude higher computation and communication cost compared to plaintext counterpart. Unlike the plaintext evaluation where non-linear operator contribute to much smaller portion of latency compared to linear operator, the MPC based encrypted evaluation of non-linear operator leads to enormous latency overhead and becomes the major bottlenecks for PI application. 

% \textcolor{blue}{How to improve MPC based private inference} \\
% \textcolor{blue}{Traditional approaches} \\
% Traditional approaches to evaluate the non-linear function for PI includes Newton-Rhapson iterations for polynomial approximation \cite{knott2021crypten}, piece-wise linear approximation \cite{lazzeretti2015piecewise}. However, those methods either needs a high degree of polynomial function or requires multiple rounds of encrypted comparison implementation, and both ways lead to a non-negligible overhead for PI application. 



% \subsubsection{Overhead Reduction of MPC Comparison Protocol.}
\subsection{Comparison Overhead Reduction Algorithms.}

% \textcolor{blue}{benefit and drawback of polynomial approximation} \\
% Existing MPC comparison protocol overhead reduction fall into three categories: \textit{ReLU (comparison) overhead reduction} by using model compression \cite{sanyal2018tapas, riazi2019xonn},  neural architecture search (NAS) for DNN model with smaller number of ReLUs \cite{aggarwal2020soteria, ghodsi2020cryptonas}, and fine-grained ReLU replacement with polynomial function \& ReLU dropping \cite{mishra2020delphi, ali2020polynomial, lou2020safenet, jha2021deepreduce}. 

TAPAS \cite{sanyal2018tapas} and XONN \cite{riazi2019xonn} compressed the model into binary neural network format which has reduced number of bits, and the method can effectively reduce the size of Garbled circuit for MPC comparison protocol implementation. CryptoNAS \cite{ghodsi2020cryptonas} and Sphynx \cite{cho2021sphynx} are two typical NAS directed works which define searched spaces with reduced count of ReLU and MaxPool and find the suitable architecture. Delphi\cite{mishra2020delphi}, SafeNet \cite{lou2020safenet}, and Cho's work~\cite{cho2022selective} focus on partially replacing ReLU function with polynomial function to achieve speedup in MPC based PI.  
However, polynomial replacement of ReLU often comes with a non-negligible model accuracy degradation. The reduction of non-polynomial operators (e.g., ReLU or maxpool) in these works still leads to a severe accuracy drop due to their frameworks' limitation, and they can not achieve comparison free PI implementation. To maintain accuracy, a low ReLU reduction ratio needs to be used. As a result, these works suffer from high latency due to limited computation and communication saving. Furthermore, none of the aforementioned methods have been validated in large scale model and dataset, such as ResNet 50 structure on ImageNet, which put a doubt on the scalability of those works. 
%Thus, reinforcement learning based neural architecture search (NAS) has also been introduced to find the NN structure which partially replace ReLU with polynomial function, which greatly alleviate the comparison protocol's overhead during PI. Featured examples includes SafeNet \cite{lou2020safenet} and Cho's work~\cite{cho2022selective}. 
%To maintain accuracy, a low reduction ratio needs to be used. As a result, these works suffer from high latency due to limited computation and communication saving.
% the performance of CryptoNAS is limited as it is featureless search target. 


% As shown in Tab.~\textcolor{red}{add table}, fully replace ReLU function with second order polynomial function can potential lead to more than \textcolor{red}{XXX} times communication overhead reduction and \textcolor{red}{XXX} times latency reduction for MPC based secure non-linear layer inference. 




% % Cryptographic NN requires 2PC comparison protocol implementation for non-polynomial layers such as ReLU and MaxPool. 
% Existing MPC comparison protocol overhead reduction fall into two categories:
% % There are 2 general research trend to reduce the 2PC comparison protocol overhead for cryptographic NN inference: 
% model compression \cite{aggarwal2020soteria, sanyal2018tapas, riazi2019xonn, ghodsi2020cryptonas, jha2021deepreduce} and polynomial approximation \cite{mishra2020delphi, ali2020polynomial, lou2020safenet}. 
% TAPAS \cite{sanyal2018tapas}, XONN \cite{riazi2019xonn}, and Soteria \cite{aggarwal2020soteria} focus on Binary Neural Network (BNN) for cryptographic inference, however, 
% % and provide unsatisfactory accuracy. Furthermore, BNN works still
% % suffering from accuracy degradation due to the extremely low bit representation of weight parameters, and high latency since the required secure comparison protocol still dominates system latency. 
% % However, 
% % the reduction of non-polynomial operators (e.g., ReLU or maxpool) leads to a severe accuracy drop. To maintain accuracy, a low reduction ratio needs to be used, as a result, these works suffer from high latency since the required secure comparison protocol still dominates system latency.
% the reduction of non-polynomial operators (e.g., ReLU or maxpool) leads to a severe accuracy drop. To maintain accuracy, a low reduction ratio needs to be used, as a result, these works suffer from high latency due to limited computational cost saving.

% CryptoNAS \cite{ghodsi2020cryptonas} utilizes reinforcement learning (RL) based micro-architecture search framework \cite{pham2018efficient} to improve the parameter to ReLU ratio and find the near-optimal structure. 
% However, the performance of CryptoNAS is limited as it is featureless search target. 
% The method is also not scalable due to the long training time incurred by RL-based search framework. 
% %  \textcolor{blue}{DeepReDuce \cite{jha2021deepreduce} proposes to conduct channel-wise ReLU pruning, and achieves a higher accuracy and ReLU reduction trade-off through NN regularization methods such as knowledge distillation. However, the DeepReDuce implementation faces a similar issue as SAFENet, i.e. communication channel building overhead. } \textcolor{red}{CD: this sentence could serve as a buffer to satisfy the page limit.}
% Delphi\cite{mishra2020delphi} and SAFENet \cite{lou2020safenet} propose to replace ReLU operation with polynomial activation. 
% %tony: to xxx ReLU operation with ....? replace, equip??
% %and achieves a high polynomial replacement ratio but 
% %with the sacrifice of model accuracy. 
% However, the reduction of ReLU operations leads to a severe accuracy drop in their implementation. 
% %account for 93\% online inference latency in Delphi's framework. 
% % SAFENet \cite{lou2020safenet} proposes a ReLU replacement framework with more fine-grained multi-degree channel-wise polynomial approximation to reduce the ReLU count. However, the high replacement ratio still leads to a high accuracy degradation. The channel-wise polynomial approximation method cannot avoid the constant communication channel building overhead \textcolor{red}{(Yukui, cite{??})} since each ReLU layer still requires a ReLU implementation.  

% % Further, existing works on reducing ReLU overhead have the following limitations: 
% % 1. Only ReLU replacement is considered in the existing work. However, MaxPool operations also require secure comparison implementation and the replacement is not discussed in previous works. 
% % 2. existing works only report performance for CIFAR-10 and CIFAR-100, not on ImageNet dataset.
% % % . No existing works reports large-scale Cryptographic NN performance on ImageNet dataset. 
% % The scalability of existing works remains unknown.
% % 3. The higher reduction ratio of ReLU operation leads to a severe accuracy degradation. 

% % Existing works \cite{ali2020polynomial, lou2020safenet} seek to replace the expensive non-polynomial layers with polynomial estimation. However, such replacement incurs significant accuracy degradation, and hence is not durable \textcolor{red}{(CD: why is not durable? Do you mean in these applications, the accuracy drop is not tolerable?)} for large-scale tasks such as image segmentation and video processing. 
% % The thought leads to an question: why not directly train the neural network using polynomial activation function? 

% % Instead of heuristically checking the model sensitivity after a DNN is well-trained, by deleting or replacing some non-polynomial layers or operators,
% % our key design principle is to {\em enforce} exactly
% % what is assumed in the DNN design---training a DNN that is both hardware efficient and secure while maintaining high accuracy. 
% % An naive solution to the target is to the directly replace the non-polynomial layers in a backbone model with the trainable polynomial one during neural network training, such as replacing MaxPool with AvgPool and replacing ReLU with second order polynomial activation function. The polynomial replacement is different from existing works \cite{mishra2020delphi, ali2020polynomial} since such models are directly trained with polynomial activation function. 

\subsection{Hardware Acceleration of Secure DNNs.}
% \textcolor{blue}{hardware acceleration approaches} \\
% The energy efficiency challenge \textcolor{red}{???} of secure DNN models motivates the second trend: {\em hardware acceleration}. 
The growing computing capability and energy efficiency of computing platforms such as CPUs, GPUs and FPGAs mitivates the second trend: {\em hardware acceleration for PI}. 
The state-of-the-art secure DNNs using MPC are mainly implemented on CPUs. For instance, CrypTFlow~\cite{kumar2020cryptflow} converts TensorFlow inference code~\cite{abadi2016tensorflow} into MPC protocols at the push of a button using Intel SGX. MP-SPDZ~\cite{keller2020mp} primarily targets at the compiler level, i.e., compile the high-level secure protocol code (bytecode) into virtual machine. CrypTFlow2~\cite{rathee2020cryptflow2} further improves CrypTFlow by using Athos, an end-to-end compiler, to convert TensorFlow to MPC protocols.
% It uses a 3.7 GHz Intel Xeon processor (CPU) consisting of 4 cores and 16 GBs of RAM.  
GAZELLE~\cite{juvekar2018gazelle} uses a combination of homomorphic encryption (HE) and traditional two-party computation techniques (such as garbled circuits) on Intel Xeon E5-2666 CPU with 7.5GB memory and demonstrates three orders of magnitude faster inference time, compared with fully homomorphic approaches such as CryptoNets~\cite{gilad2016cryptonets}. 
%Prior arts mainly focus on CPU (e.g., CrypTFlow~\cite{kumar2020cryptflow}, MP-SPDZ~\cite{keller2020mp}, GAZELLE~\cite{juvekar2018gazelle}) and GPU (e.g., CryptGPU~\cite{tan2021cryptgpu}) implementations. 

Recently, a DNN system built on graphics processing unit ({GPU}) using MPC, titled CryptGPU~\cite{tan2021cryptgpu}, has been discussed. 
%has drawn attention from both academia and industry. 
CryptGPU embeds cryptographic operations over secret-shared values into the floating-point operations for CUDA kernels. It achieves up to 150$\times$ speedups over CPU-based solutions. Later, CryptGPU work is incorporate into Crypten framework~\cite{knott2021crypten} to enable easy to use pytorch-based MPC framework with GPU acceleration backend. 
%CryptGPU could provide up to 150$\times$ faster than CPU-based designs. 

% However, prior works are power-hungry. For example, our observation shows that, CrpytGPU \cite{tan2021cryptgpu} requires $(700W \cdot 9.44s)$ power and over 2.7GB communication size to run the MPC-based VGG16 network.
% Later, CryptGPU work is incorporate into Crypten framework~\cite{knott2021crypten} to enable easy to use pytorch-based MPC framework with GPU acceleration backend. 
%In this work, we build an end-to-end MPC based PI framework on FPGAs as the first effort, and we thoroughly investigate secret sharing MPC protocol's overhead for PI application.

% Secure MPC, a cryptographic technique, is used to allow multiple parties to jointly and securely perform a function while keeping each party's inputs private. MPC is capable of providing security guarantees as robust as those achievable by trusted third parties~\cite{canetti2001universally}. 
% % For instance, with absolutely no information is leaked other than that can be obtained from the expected function outputs.
% Researchers have been using MPC to build secure, privacy-preserving DNN frameworks. The state-of-the-art secure DNNs using MPC are mainly implemented on CPUs. For instance, CrypTFlow~\cite{kumar2020cryptflow} converts TensorFlow inference code~\cite{abadi2016tensorflow} into MPC protocols at the push of a button using Intel SGX. MP-SPDZ~\cite{keller2020mp} primarily targets at the compiler level, i.e., compile the high-level secure protocol code (bytecode) into virtual machine. CrypTFlow2~\cite{rathee2020cryptflow2} further improves CrypTFlow by using Athos, an end-to-end compiler, to convert TensorFlow to MPC protocols.
% % It uses a 3.7 GHz Intel Xeon processor (CPU) consisting of 4 cores and 16 GBs of RAM.  
% GAZELLE~\cite{juvekar2018gazelle} uses a combination of homomorphic encryption (HE) and traditional two-party computation techniques (such as garbled circuits) on Intel Xeon E5-2666 CPU with 7.5GB memory and demonstrates three orders of magnitude faster inference time, compared with fully homomorphic approaches such as CryptoNets~\cite{gilad2016cryptonets}. 

% Recently, a DNN system built on graphics processing unit ({GPU}) using MPC, titled CryptGPU~\cite{tan2021cryptgpu}, has been discussed. 
% %has drawn attention from both academia and industry. 
% CryptGPU embeds cryptographic operations over secret-shared values into the floating-point operations for CUDA kernels. It achieves up to 150$\times$ speedups over CPU-based solutions. 
% % In the past decades, various practical constructions have been proposed that reduce the security guarantees to the computational hardness assumption~\cite{yao1986generate, lindell2009proof}, the honest majority~\cite{ben2019completeness, beaver1991secure}, and the availability of correlated randomness~\cite{beaver1996correlated}. Recently, several general MPC frameworks~\cite{demmler2015aby, patra2021aby2} have been proposed to enhance the practicality of the state-of-the-art MPC algorithms.  

% \subsection{Our Hardware Aware NAS Framework}
% \textcolor{red}{add our framework description}

% \subsection{Threat Model}

% % \textcolor{red}{Copied from MICRO, rewrite,@Ranran, Nuo}
% % \noindent\textbf{Two ``servers'' setup.} 
% % In this work, we consider the generic secure computing framework that leverages two  non-colluding computing ``servers''~\cite{demmler2015aby, kamara2011outsourcing}. Such secure computing setup is typically used to design client-server applications (i.e. MLaaS). In this scheme, the client secretly outsources their confidential input to two computing servers. The servers then invoke a 
% % two party secure computing protocol to securely evaluate a function with user submitted inputs. The 2PC protocol ensures that the servers are unaware of the intermediate information, and the computed outputs. It is worth noting that this server-aided secure computation set up can be used for general multi-party applications as well, where an arbitrary number of clients provide their confidential inputs~\cite{demmler2015aby}.

% \noindent\textbf{2PC setup.} 
% % In this work, we consider a generic secure computing framework commonly used in client-server applications (i.e., MLaaS) that utilizes two non-colluding computing ``servers'' 
% We consider a similar scheme involving two semi-honest in a MLaaS applications~\cite{demmler2015aby, kamara2011outsourcing}.
% % in a MLaaS application proposed in previous work~\cite{demmler2015aby, kamara2011outsourcing}. 
% In this scheme, the two servers receive the confidential inputs that are secretly outsourced from the client and invoke a two party secure computing protocol to securely evaluate the function within the given inputs. The 2PC protocol ensures that intermediate information and computation results are not exposed to the servers during the evaluation process. Notably, this server-aided secure computation setup could also be used for an arbitrary number of clients, providing their confidential inputs for general multi-party applications ~\cite{demmler2015aby}.

% \vspace{1mm}
% \noindent\textbf{Threat model.} 
% % We consider an adversary who corrupts computing servers to launch attacks. Specifically, we consider an {\it admissible adversary}~\cite{mohassel2017secureml} who is able to corrupt at most one server at a time. This assumption captures the {\it non-colluding server} setup. Additionally, we focus on the honest but curious model where the adversary does not deviate from the protocol specification, but can do arbitrary side computations in an attempt to violate the system's security. 
% We assume that an {\it admissible adversary}~\cite{mohassel2017secureml} who can compromise up to one server at a time to launch attacks,
% which captures the {\it non-colluding server} assumption. 
% Furthermore, we focus on a semi-honest security model~\cite{patra2021aby2,choi2019hybrid,husted2013gpu,zhang2013picco} where the adversary is "honest but curious", which does not deviate from the protocol specification but can do arbitrary side calculations that try to violate the security of the system.
% Although this is not the strongest assumption, this model makes sense in the context of many real-world applications, 
% as simply starting a secure computing instance already requires a substantial degree of trust between all parties.
% % as simply starting an instance of a secure computation would already require a substantial degree of trust among all parties. 



% % \subsection{Cryptographic Building Blocks}
% % \section{Hardware Acceleration for Secure DNNs}
% % \section{Cryptographic Hardware Acc. }

==> sections/A_suggestion.tex <==
\section{Suggestion}
\textcolor{blue}{
0. Profiling X2act latency and ReLU latency \\
1. Convergence prove of x2act: YiJue. \\
2. Normalized latency comparison of ReLU and X (LAN and WAN): YuKui \\
3. Contribution of x2act training, how to set the parameter to be trainble, how to make show it does not explode, reference: POLYNOMIAL ACTIVATION FUNCTIONS 
\url{https://openreview.net/attachment?id=rkxsgkHKvH&name=original_pdf}\\
4. training process: gradually replacement. reference: AdderNet
\url{https://arxiv.org/pdf/2105.14202.pdf}\\
5. Contribution of quantization: Nuo Xu\\
6. Multi-FPGA client with single GPU server experiment? GPU virtualization\\
7. 2 edge FPGA setting? energy efficiency\\
8. 2 FPGA U280? low latency + energy efficiency at low batch size\\
9. 2 GPU for low latency comaprison at large batch size(GPU can use Crypten)?\\
10. FPGA <-> GPU performance comparison: latency vs. batch size on different model. \\
11. Profiling wrap around error, get a (model accuracy) <-> (end to end ss ring bit width) trade off. \\
12. Activation Sparsification (CSR format overhead)\\
Major contribution: \\
1. Why we are able to converge with polynomial replacement? Initialize $w0 = 0$, $w1 = 1$ for $w0x^2 + w1 x$, can converge better, proof from Yijue. Polynomial replacement policy (post-training replacement \\
2. Layer-wise (including activation function) coarse-grained pipeline including network latency and hardware resource. Use layer-wise latency for NAS. Reference: NAAS @Songhan, FPGA-Implementation Aware Neural Architecture Search @weiwen jiang\\
3. Explore possibility for aggressive quantization,  \\
4. Activation sparsity. 
5. Hide network latency through coarse-grained pipeline (dataflow architecture, producer: Con2D tile computation, consumer: tile communication network)
}



\cw{general paradigm/auto framework for efficient on-linear optimization.}

\cw{You could argue that existing methods usually require approximating nonlinear operators with high-order polynomials or using piece-wise approximation techniques, which can be heavyweight for achieving high accuracy. Our approach replaces the non-linear operations with a low-degree polynomial and does not require piece-wise approximation techniques. Say something that this approach is efficient in energy or power, etc.}

\cw{You may present your simulation as one approach under this general idea, and there may exists many other methods. Thus our paradigm provides an template for innovating better algorithms, i.e. one may utilizes optimized approaches to find the replacement activation functions.}
\textcolor{red}{framework, to change relu to polynomial, paradigm. Add hardware latency + accuracy constriant search, search a optimal neural network . we only add a fpga test case, method can be extend to other platform. }
